Towards Purely Unsupervised Disentanglement of Appearance and Shape for Person Images Generation

There have been a fairly of research interests in exploring the disentanglement of appearance and shape from human images. Most existing endeavours pursuit this goal by either using training images with annotations or regulating the training process with external clues such as human skeleton, body segmentation or cloth patches etc. In this paper, we aim to address this challenge in a more unsupervised manner---we do not require any annotation nor any external task-specific clues. To this end, we formulate an encoder-decoder-like network to extract both the shape and appearance features from input images at the same time, and train the parameters by three losses: feature adversarial loss, color consistency loss and reconstruction loss. The feature adversarial loss mainly impose little to none mutual information between the extracted shape and appearance features, while the color consistency loss is to encourage the invariance of person appearance conditioned on different shapes. More importantly, our unsupervised (Unsupervised learning has many interpretations in different tasks. To be clear, in this paper, we refer unsupervised learning as learning without task-specific human annotations, pairs or any form of weak supervision.) framework utilizes learned shape features as masks which are applied to the input itself in order to obtain clean appearance features. Without using fixed input human skeleton, our network better preserves the conditional human posture while requiring less supervision. Experimental results on DeepFashion and Market1501 demonstrate that the proposed method achieves clean disentanglement and is able to synthesis novel images of comparable quality with state-of-the-art weakly-supervised or even supervised methods.

==> Sec4_ImplementationDetail.tex <==
\vspace{-2mm}
\section{Datasets \& Implementation Details}
\subsection{Datasets}
In order to show the versatility of the proposed method, we test the network on two very different datasets: DeepFashion \cite{liuLQWTcvpr16DeepFashion} for human images and CK+ \cite{lucey2010extended} for faces.

\vspace{-4mm}
\paragraph{DeepFashion}
We use the In-shop Clothes Retrieval Benchmark of DeepFashion which contains 52712 of in-shop clothes images. The dataset offers various different clothes on many different persons. All back-view images are filtered out because it is hard to distinguish between back-view and front-view based on pose images. Including back-view ones will result in training instability. We use OpenPose \cite{cao2017realtime} to extract poses for each image prior to training our network because the pose keypoints are not given for this dataset. We configure Openpose to use the \emph{COCO} model, which outputs 18 keypoints.

\vspace{-4mm}
\paragraph{CK+}
The CK+ dataset has 10701 frames of different facial expressions performed by different persons. Every frame is FACS coded and comes with 68 landmarks annotation. This being a video dataset, image pairs of the the same person in different facial expressions are available. However, we do not exploit such paired information and treat each frame as an independent image.

\vspace{-2mm}
\subsection{Implementation Details}
The network is optimized using Adam optimizer \cite{kingma2014adam} with initial learning rate of 0.0002, $\beta_1=0.9$ and $\beta_2=0.999$. The learning rate is decreased by 10\% every 2000 iterations. The batch size is set to 16 primarily due to hardware limitations. We update the generator and the discriminators alternately on every step. Also the hyper-parameters in Eq~\ref{Eq:full_loss} are simply set to 1, which we find to be good enough. This also indicates the simplicity of the model because little parameter tuning is required. The full details of the network structure is given in the supplementary material.

Since our goal is unsupervised image generation and representation learning, we do not define image level train-test splits. Instead, we distinguish training and testing on appearance-pose image pairs. This is easy to accomplish because there exits a tremendous amount of such random pairs for each dataset. \TZ{Hongtao, Write some GPU and machine details, and indicate whether using tensorflow or pytorch.}
